Data Poisoning Attacks on Regression Learning and Corresponding Defenses

Adversarial data poisoning is an effective attack against machine learning and threatens model integrity by introducing poisoned data into the training dataset. So far, it has been studied mostly for classification, even though regression learning is used in many mission critical systems (such as dosage of medication, control of cyber-physical systems and managing power supply). Therefore, in the present research, we aim to evaluate all aspects of data poisoning attacks on regression learning, exceeding previous work both in terms of breadth and depth. We present realistic scenarios in which data poisoning attacks threaten production systems and introduce a novel black-box attack, which is then applied to a real-word medical use-case. As a result, we observe that the mean squared error (MSE) of the regressor increases to 150 percent due to inserting only two percent of poison samples. Finally, we present a new defense strategy against the novel and previous attacks and evaluate it thoroughly on 26 datasets. As a result of the conducted experiments, we conclude that the proposed defence strategy effectively mitigates the considered attacks.

==> possible_conferences.tex <==
| 110 | ECIR 2021                         | Oct 1, 2020                 | B, A2, | Mar 28, 2021 - Apr 1, 2021  | European Conference on Information Retrieval                                             | Lucca, Italy              |   nan |
|   0 | PRDC 2020             | Jul 18, 2020                | B, B1, | Dec 1, 2020 - Dec 4, 2020   | The 25th IEEE Pacific Rim International Symposium on Dependable Computing                                  | Perth, Australia                 |   nan |


==> resources/all_results.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
           &      &  \_mse\_\_poison\_flip &  \_mse\_\_poison\_flip/defense\_itrim &  \_mse\_\_poison\_flip/defense\_trim &  \_mse\_\_poison\_flip/epshat-eps &  \_mse\_\_poison\_statP &  \_mse\_clean &  eps\_hat \\
data & eps &                    &                                  &                                 &                               &                     &             &          \\
\midrule
ANACALT.dat & 0.00 &           0.032206 &                         0.041167 &                        0.045722 &                          0.10 &            0.030725 &    0.029692 &     0.14 \\
           & 0.02 &           0.032214 &                         0.040737 &                        0.045849 &                          0.08 &            0.032211 &    0.031666 &     0.14 \\
           & 0.04 &           0.033563 &                         0.042150 &                        0.042150 &                          0.10 &            0.035983 &    0.031498 &     0.14 \\
           & 0.06 &           0.035869 &                         0.038038 &                        0.038038 &                          0.08 &            0.035575 &    0.032252 &     0.14 \\
           & 0.08 &           0.038477 &                         0.035923 &                        0.038761 &                          0.06 &            0.036909 &    0.032189 &     0.14 \\
           & 0.10 &           0.040359 &                         0.032829 &                        0.034501 &                          0.04 &            0.038075 &    0.031439 &     0.14 \\
accel & 0.00 &           0.002302 &                         0.002302 &                        0.003133 &                          0.00 &            0.002301 &    0.002301 &     0.14 \\
           & 0.02 &           0.005654 &                         0.002584 &                        0.002795 &                          0.00 &            0.004283 &    0.002684 &     0.14 \\
           & 0.04 &           0.011037 &                         0.002183 &                        0.002479 &                          0.00 &            0.004609 &    0.002265 &     0.14 \\
           & 0.06 &           0.018555 &                         0.002877 &                        0.003187 &                          0.00 &            0.005052 &    0.002852 &     0.14 \\
           & 0.08 &           0.014831 &                         0.002596 &                        0.002730 &                          0.00 &            0.005369 &    0.002594 &     0.14 \\
           & 0.10 &           0.020462 &                         0.002414 &                        0.002547 &                          0.00 &            0.006893 &    0.002556 &     0.14 \\
ailerons.dat & 0.00 &           0.002624 &                         0.002462 &                        0.002874 &                          0.00 &            0.002486 &    0.002590 &     0.14 \\
           & 0.02 &           0.003715 &                         0.002449 &                        0.002742 &                          0.00 &            0.002890 &    0.002423 &     0.14 \\
           & 0.04 &           0.005999 &                         0.002521 &                        0.002724 &                          0.00 &            0.003312 &    0.002522 &     0.14 \\
           & 0.06 &           0.008470 &                         0.002541 &                        0.002639 &                          0.00 &            0.004179 &    0.002541 &     0.14 \\
           & 0.08 &           0.012111 &                         0.002493 &                        0.002798 &                          0.00 &            0.003720 &    0.002567 &     0.14 \\
           & 0.10 &           0.015327 &                         0.002537 &                        0.002611 &                          0.00 &            0.004563 &    0.002563 &     0.14 \\
armesHousing & 0.00 &           0.003852 &                         0.003852 &                        0.003438 &                          0.00 &            0.003852 &    0.003852 &     0.14 \\
           & 0.02 &           0.005887 &                         0.002521 &                        0.004020 &                          0.00 &            0.004231 &    0.002072 &     0.14 \\
           & 0.04 &           0.006308 &                         0.003547 &                        0.004399 &                          0.02 &            0.008517 &    0.003560 &     0.14 \\
           & 0.06 &           0.014838 &                         0.004715 &                        0.006348 &                          0.00 &            0.010023 &    0.004276 &     0.14 \\
           & 0.08 &           0.016888 &                         0.002655 &                        0.003452 &                          0.00 &            0.010149 &    0.002169 &     0.14 \\
           & 0.10 &           0.016037 &                         0.003122 &                        0.003603 &                          0.02 &            0.009562 &    0.002018 &     0.14 \\
availPwr & 0.00 &           0.001080 &                         0.001080 &                        0.001344 &                          0.00 &            0.001075 &    0.001075 &     0.14 \\
           & 0.02 &           0.003547 &                         0.001323 &                        0.002239 &                          0.00 &            0.003589 &    0.001330 &     0.14 \\
           & 0.04 &           0.006825 &                         0.001314 &                        0.002207 &                          0.00 &            0.005466 &    0.001315 &     0.14 \\
           & 0.06 &           0.010493 &                         0.002260 &                        0.001825 &                          0.00 &            0.006897 &    0.000990 &     0.14 \\
           & 0.08 &           0.013583 &                         0.002260 &                        0.001951 &                          0.00 &            0.008575 &    0.001091 &     0.14 \\
           & 0.10 &           0.019895 &                         0.003638 &                        0.001386 &                          0.00 &            0.010491 &    0.001079 &     0.14 \\
bank8fm & 0.00 &           0.002503 &                         0.002503 &                        0.002654 &                          0.00 &            0.002503 &    0.002483 &     0.14 \\
           & 0.02 &           0.003861 &                         0.002400 &                        0.002508 &                          0.00 &            0.003820 &    0.002430 &     0.14 \\
           & 0.04 &           0.006575 &                         0.002337 &                        0.002449 &                          0.00 &            0.007104 &    0.002364 &     0.14 \\
           & 0.06 &           0.010367 &                         0.002398 &                        0.002627 &                          0.00 &            0.010260 &    0.002508 &     0.14 \\
           & 0.08 &           0.014543 &                         0.002342 &                        0.002371 &                          0.00 &            0.013077 &    0.002543 &     0.14 \\
           & 0.10 &           0.019490 &                         0.002400 &                        0.002531 &                          0.00 &            0.010372 &    0.002392 &     0.14 \\
california.dat & 0.00 &           0.018781 &                         0.019531 &                        0.020022 &                          0.08 &            0.018781 &    0.018781 &     0.14 \\
           & 0.02 &           0.020817 &                         0.020114 &                        0.021172 &                          0.08 &            0.022066 &    0.019448 &     0.14 \\
           & 0.04 &           0.023845 &                         0.019394 &                        0.020277 &                          0.08 &            0.024904 &    0.019002 &     0.14 \\
           & 0.06 &           0.028551 &                         0.021505 &                        0.021505 &                          0.08 &            0.024577 &    0.021032 &     0.14 \\
           & 0.08 &           0.030271 &                         0.020442 &                        0.020442 &                          0.06 &            0.023395 &    0.020009 &     0.14 \\
           & 0.10 &           0.032602 &                         0.021613 &                        0.021181 &                          0.04 &            0.027547 &    0.020517 &     0.14 \\
compactiv.dat & 0.00 &           0.008949 &                         0.021508 &                        0.023445 &                          0.02 &            0.009032 &    0.009032 &     0.14 \\
           & 0.02 &           0.009817 &                         0.024153 &                        0.028190 &                          0.02 &            0.011023 &    0.009184 &     0.14 \\
           & 0.04 &           0.014466 &                         0.032833 &                        0.029606 &                          0.02 &            0.013477 &    0.008398 &     0.14 \\
           & 0.06 &           0.015248 &                         0.029575 &                        0.028237 &                          0.00 &            0.019979 &    0.009267 &     0.14 \\
           & 0.08 &           0.021913 &                         0.032546 &                        0.027755 &                          0.00 &            0.019721 &    0.008392 &     0.14 \\
           & 0.10 &           0.023761 &                         0.031351 &                        0.030771 &                          0.00 &            0.009279 &    0.009237 &     0.14 \\
concrete.dat & 0.00 &           0.016196 &                         0.030261 &                        0.027382 &                          0.08 &            0.016196 &    0.016196 &     0.14 \\
           & 0.02 &           0.017488 &                         0.030563 &                        0.029492 &                          0.08 &            0.017627 &    0.016186 &     0.14 \\
           & 0.04 &           0.019941 &                         0.020213 &                        0.025402 &                          0.06 &            0.022051 &    0.016942 &     0.14 \\
           & 0.06 &           0.021436 &                         0.017183 &                        0.017518 &                          0.06 &            0.022063 &    0.016186 &     0.14 \\
           & 0.08 &           0.024771 &                         0.017574 &                        0.017699 &                          0.06 &            0.027965 &    0.016234 &     0.14 \\
           & 0.10 &           0.027099 &                         0.017310 &                        0.017310 &                          0.04 &            0.030279 &    0.017125 &     0.14 \\
cpu & 0.00 &           0.009592 &                         0.011996 &                        0.018135 &                          0.02 &            0.009592 &    0.009592 &     0.14 \\
           & 0.02 &           0.010516 &                         0.027701 &                        0.025975 &                          0.02 &            0.008124 &    0.008130 &     0.14 \\
           & 0.04 &           0.013634 &                         0.033745 &                        0.030104 &                          0.02 &            0.013125 &    0.008580 &     0.14 \\
           & 0.06 &           0.019475 &                         0.034063 &                        0.034240 &                          0.00 &            0.011615 &    0.010020 &     0.14 \\
           & 0.08 &           0.020561 &                         0.032259 &                        0.032207 &                          0.00 &            0.009816 &    0.006794 &     0.14 \\
           & 0.10 &           0.026061 &                         0.036500 &                        0.033821 &                          0.00 &            0.026991 &    0.010332 &     0.14 \\
elevators.dat & 0.00 &           0.001805 &                         0.001824 &                        0.001927 &                          0.00 &            0.001805 &    0.001824 &     0.14 \\
           & 0.02 &           0.003047 &                         0.001953 &                        0.002147 &                          0.00 &            0.003207 &    0.001950 &     0.14 \\
           & 0.04 &           0.005120 &                         0.001770 &                        0.001955 &                          0.00 &            0.002660 &    0.001890 &     0.14 \\
           & 0.06 &           0.008221 &                         0.001992 &                        0.002232 &                          0.00 &            0.004340 &    0.001989 &     0.14 \\
           & 0.08 &           0.011251 &                         0.002123 &                        0.002262 &                          0.00 &            0.004749 &    0.001939 &     0.14 \\
           & 0.10 &           0.014370 &                         0.001863 &                        0.001970 &                          0.00 &            0.004389 &    0.001919 &     0.14 \\
friedman.dat & 0.00 &           0.009100 &                         0.009057 &                        0.009235 &                          0.02 &            0.009100 &    0.008859 &     0.14 \\
           & 0.02 &           0.009452 &                         0.009147 &                        0.009148 &                          0.02 &            0.009731 &    0.009094 &     0.14 \\
           & 0.04 &           0.010953 &                         0.009147 &                        0.009283 &                          0.02 &            0.009953 &    0.007896 &     0.14 \\
           & 0.06 &           0.010895 &                         0.008256 &                        0.008300 &                          0.02 &            0.009930 &    0.008146 &     0.14 \\
           & 0.08 &           0.014246 &                         0.008352 &                        0.008445 &                          0.02 &            0.012357 &    0.008064 &     0.14 \\
           & 0.10 &           0.018773 &                         0.008342 &                        0.008967 &                          0.02 &            0.013807 &    0.008344 &     0.14 \\
fuelCons & 0.00 &           0.001556 &                         0.001556 &                        0.002047 &                          0.00 &            0.001556 &    0.001556 &     0.14 \\
           & 0.02 &           0.004859 &                         0.003398 &                        0.003315 &                          0.00 &            0.003751 &    0.002002 &     0.14 \\
           & 0.04 &           0.008468 &                         0.001934 &                        0.002304 &                          0.00 &            0.004785 &    0.001662 &     0.14 \\
           & 0.06 &           0.009866 &                         0.002198 &                        0.002809 &                          0.00 &            0.006698 &    0.001884 &     0.14 \\
           & 0.08 &           0.015469 &                         0.002528 &                        0.003442 &                          0.00 &            0.006332 &    0.001468 &     0.14 \\
           & 0.10 &           0.017499 &                         0.002592 &                        0.002730 &                          0.00 &            0.011993 &    0.001950 &     0.14 \\
heat & 0.00 &           0.002415 &                         0.002415 &                        0.003306 &                          0.00 &            0.002415 &    0.002415 &     0.14 \\
           & 0.02 &           0.004503 &                         0.002538 &                        0.003537 &                          0.00 &            0.002887 &    0.002511 &     0.14 \\
           & 0.04 &           0.008604 &                         0.002475 &                        0.003579 &                          0.00 &            0.002936 &    0.002381 &     0.14 \\
           & 0.06 &           0.012169 &                         0.002487 &                        0.003148 &                          0.00 &            0.003183 &    0.002484 &     0.14 \\
           & 0.08 &           0.017337 &                         0.002527 &                        0.003293 &                          0.00 &            0.003350 &    0.002623 &     0.14 \\
           & 0.10 &           0.023861 &                         0.002842 &                        0.003366 &                          0.00 &            0.003139 &    0.002759 &     0.14 \\
house.dat & 0.00 &           0.007658 &                         0.007952 &                        0.009294 &                          0.02 &            0.007567 &    0.007567 &     0.14 \\
           & 0.02 &           0.007844 &                         0.007911 &                        0.008336 &                          0.02 &            0.007606 &    0.007433 &     0.14 \\
           & 0.04 &           0.009754 &                         0.008179 &                        0.008587 &                          0.02 &            0.010352 &    0.007722 &     0.14 \\
           & 0.06 &           0.011444 &                         0.006930 &                        0.008296 &                          0.02 &            0.014188 &    0.006889 &     0.14 \\
           & 0.08 &           0.014480 &                         0.007932 &                        0.008314 &                          0.02 &            0.015246 &    0.007475 &     0.14 \\
           & 0.10 &           0.018244 &                         0.007569 &                        0.007772 &                          0.02 &            0.012948 &    0.007241 &     0.14 \\
loan & 0.00 &           0.002757 &                         0.002757 &                        0.002928 &                          0.00 &            0.002757 &    0.002757 &     0.14 \\
           & 0.02 &           0.005036 &                         0.003150 &                        0.008112 &                          0.00 &            0.004449 &    0.002745 &     0.14 \\
           & 0.04 &           0.008613 &                         0.003158 &                        0.009190 &                          0.00 &            0.005969 &    0.002787 &     0.14 \\
           & 0.06 &           0.013032 &                         0.003061 &                        0.007018 &                          0.00 &            0.006955 &    0.002693 &     0.14 \\
           & 0.08 &           0.016514 &                         0.003203 &                        0.005994 &                          0.00 &            0.008362 &    0.002649 &     0.14 \\
           & 0.10 &           0.022463 &                         0.003238 &                        0.004719 &                          0.00 &            0.009128 &    0.002701 &     0.14 \\
mortgage.dat & 0.00 &           0.000075 &                         0.000075 &                        0.000099 &                          0.00 &            0.000075 &    0.000075 &     0.14 \\
           & 0.02 &           0.001988 &                         0.000217 &                        0.000337 &                          0.00 &            0.001927 &    0.000216 &     0.14 \\
           & 0.04 &           0.006508 &                         0.000104 &                        0.000142 &                          0.00 &            0.003516 &    0.000217 &     0.14 \\
           & 0.06 &           0.012371 &                         0.000113 &                        0.000148 &                          0.00 &            0.005160 &    0.000187 &     0.14 \\
           & 0.08 &           0.014011 &                         0.000089 &                        0.000111 &                          0.00 &            0.006316 &    0.000164 &     0.14 \\
           & 0.10 &           0.019512 &                         0.000116 &                        0.000168 &                          0.00 &            0.012792 &    0.000492 &     0.14 \\
plastic.dat & 0.00 &           0.021716 &                         0.022413 &                        0.022587 &                          0.10 &            0.021716 &    0.021716 &     0.14 \\
           & 0.02 &           0.024266 &                         0.025017 &                        0.025436 &                          0.10 &            0.028053 &    0.023952 &     0.14 \\
           & 0.04 &           0.023449 &                         0.022361 &                        0.022344 &                          0.10 &            0.079236 &    0.022242 &     0.14 \\
           & 0.06 &           0.024285 &                         0.024304 &                        0.024304 &                          0.08 &            0.077903 &    0.024365 &     0.14 \\
           & 0.08 &           0.027903 &                         0.021596 &                        0.021596 &                          0.06 &            0.065430 &    0.023911 &     0.14 \\
           & 0.10 &           0.032888 &                         0.022517 &                        0.022517 &                          0.04 &            0.054091 &    0.021650 &     0.14 \\
pole.dat & 0.00 &           0.089331 &                         0.101146 &                        0.101146 &                          0.14 &            0.089331 &    0.089331 &     0.14 \\
           & 0.02 &           0.090083 &                         0.098729 &                        0.098729 &                          0.12 &            0.091975 &    0.089368 &     0.14 \\
           & 0.04 &           0.091751 &                         0.097464 &                        0.097464 &                          0.10 &            0.095840 &    0.090295 &     0.14 \\
           & 0.06 &           0.092375 &                         0.097492 &                        0.097492 &                          0.08 &            0.100443 &    0.091577 &     0.14 \\
           & 0.08 &           0.091982 &                         0.093593 &                        0.093593 &                          0.06 &            0.102566 &    0.088696 &     0.14 \\
           & 0.10 &           0.094032 &                         0.091708 &                        0.091708 &                          0.04 &            0.110511 &    0.089368 &     0.14 \\
quake.dat & 0.00 &           0.032242 &                         0.033556 &                        0.033556 &                          0.14 &            0.032523 &    0.032401 &     0.14 \\
           & 0.02 &           0.031745 &                         0.033179 &                        0.033179 &                          0.12 &            0.031722 &    0.032072 &     0.14 \\
           & 0.04 &           0.031739 &                         0.033068 &                        0.033068 &                          0.10 &            0.032522 &    0.031446 &     0.14 \\
           & 0.06 &           0.032926 &                         0.035729 &                        0.035729 &                          0.08 &            0.033765 &    0.033770 &     0.14 \\
           & 0.08 &           0.033419 &                         0.035805 &                        0.035805 &                          0.06 &            0.036309 &    0.034468 &     0.14 \\
           & 0.10 &           0.035416 &                         0.032335 &                        0.032335 &                          0.04 &            0.035160 &    0.030756 &     0.14 \\
rings & 0.00 &           0.006314 &                         0.005994 &                        0.006229 &                          0.02 &            0.006234 &    0.006234 &     0.14 \\
           & 0.02 &           0.009114 &                         0.006945 &                        0.007632 &                          0.02 &            0.007981 &    0.006556 &     0.14 \\
           & 0.04 &           0.011032 &                         0.006658 &                        0.007101 &                          0.02 &            0.009255 &    0.006556 &     0.14 \\
           & 0.06 &           0.015438 &                         0.006819 &                        0.007023 &                          0.02 &            0.009720 &    0.006398 &     0.14 \\
           & 0.08 &           0.017181 &                         0.006698 &                        0.007199 &                          0.02 &            0.008989 &    0.006520 &     0.14 \\
           & 0.10 &           0.017839 &                         0.007199 &                        0.007271 &                          0.02 &            0.011254 &    0.006763 &     0.14 \\
torque & 0.00 &           0.000442 &                         0.000442 &                        0.000590 &                          0.00 &            0.000442 &    0.000442 &     0.14 \\
           & 0.02 &           0.004056 &                         0.001539 &                        0.003573 &                          0.00 &            0.003719 &    0.000590 &     0.14 \\
           & 0.04 &           0.007063 &                         0.001024 &                        0.002140 &                          0.00 &            0.005596 &    0.000945 &     0.14 \\
           & 0.06 &           0.012175 &                         0.000938 &                        0.001822 &                          0.00 &            0.009420 &    0.000818 &     0.14 \\
           & 0.08 &           0.011914 &                         0.001283 &                        0.002005 &                          0.00 &            0.011957 &    0.003378 &     0.14 \\
           & 0.10 &           0.019760 &                         0.001063 &                        0.000871 &                          0.00 &            0.011472 &    0.000671 &     0.14 \\
treasury.dat & 0.00 &           0.000245 &                         0.000249 &                        0.000269 &                          0.00 &            0.000259 &    0.000259 &     0.14 \\
           & 0.02 &           0.002538 &                         0.000167 &                        0.000162 &                          0.00 &            0.002003 &    0.000205 &     0.14 \\
           & 0.04 &           0.007179 &                         0.000212 &                        0.000229 &                          0.00 &            0.003972 &    0.000215 &     0.14 \\
           & 0.06 &           0.010939 &                         0.000190 &                        0.000201 &                          0.00 &            0.005189 &    0.000252 &     0.14 \\
           & 0.08 &           0.016623 &                         0.000247 &                        0.000251 &                          0.00 &            0.006415 &    0.000368 &     0.14 \\
           & 0.10 &           0.023044 &                         0.000238 &                        0.000220 &                          0.00 &            0.004568 &    0.000341 &     0.14 \\
wankara.dat & 0.00 &           0.000478 &                         0.000478 &                        0.000479 &                          0.00 &            0.000478 &    0.000478 &     0.14 \\
           & 0.02 &           0.002816 &                         0.000504 &                        0.000578 &                          0.00 &            0.001948 &    0.000501 &     0.14 \\
           & 0.04 &           0.005195 &                         0.000509 &                        0.000521 &                          0.00 &            0.002825 &    0.000506 &     0.14 \\
           & 0.06 &           0.009299 &                         0.000484 &                        0.000489 &                          0.00 &            0.003868 &    0.000567 &     0.14 \\
           & 0.08 &           0.013491 &                         0.000533 &                        0.000561 &                          0.00 &            0.012861 &    0.000630 &     0.14 \\
           & 0.10 &           0.014252 &                         0.000481 &                        0.000471 &                          0.00 &            0.016404 &    0.000507 &     0.14 \\
warfarin & 0.00 &           0.002820 &                         0.002820 &                        0.002900 &                          0.00 &            0.002820 &    0.002820 &     0.14 \\
           & 0.02 &           0.003463 &                         0.002694 &                        0.002760 &                          0.00 &            0.003866 &    0.002408 &     0.14 \\
           & 0.04 &           0.004877 &                         0.002383 &                        0.002474 &                          0.00 &            0.005231 &    0.002388 &     0.14 \\
           & 0.06 &           0.007638 &                         0.002532 &                        0.002640 &                          0.00 &            0.007828 &    0.002546 &     0.14 \\
           & 0.08 &           0.011723 &                         0.003044 &                        0.003000 &                          0.00 &            0.007746 &    0.002579 &     0.14 \\
           & 0.10 &           0.015159 &                         0.002994 &                        0.003059 &                          0.00 &            0.008359 &    0.002811 &     0.14 \\
wizmir.dat & 0.00 &           0.000467 &                         0.000467 &                        0.000468 &                          0.00 &            0.000466 &    0.000466 &     0.14 \\
           & 0.02 &           0.002267 &                         0.000509 &                        0.000562 &                          0.00 &            0.002277 &    0.000509 &     0.14 \\
           & 0.04 &           0.005499 &                         0.000438 &                        0.000446 &                          0.00 &            0.003358 &    0.000465 &     0.14 \\
           & 0.06 &           0.007247 &                         0.000447 &                        0.000450 &                          0.00 &            0.005901 &    0.000524 &     0.14 \\
           & 0.08 &           0.012592 &                         0.000491 &                        0.000520 &                          0.00 &            0.015139 &    0.000491 &     0.14 \\
           & 0.10 &           0.015073 &                         0.000491 &                        0.000514 &                          0.00 &            0.014745 &    0.000491 &     0.14 \\
\bottomrule
\end{tabular}

